Efficiency of Non-Truthful Auctions in Auto-bidding with Budget Constraints

We study the efficiency of non-truthful auctions for auto-bidders with both return on spend (ROS) and budget constraints. The efficiency of a mechanism is measured by the price of anarchy (PoA), which is the worst case ratio between the liquid welfare of any equilibrium and the optimal (possibly randomized) allocation. Our first main result is that the first-price auction (FPA) is optimal, among deterministic mechanisms, in this setting. Without any assumptions, the PoA of FPA is $n$ which we prove is tight for any deterministic mechanism. However, under a mild assumption that a bidder's value for any query does not exceed their total budget, we show that the PoA is at most $2$. This bound is also tight as it matches the optimal PoA without a budget constraint. We next analyze two randomized mechanisms: randomized FPA (rFPA) and "quasi-proportional" FPA. We prove two results that highlight the efficacy of randomization in this setting. First, we show that the PoA of rFPA for two bidders is at most $1.8$ without requiring any assumptions. This extends prior work which focused only on an ROS constraint. Second, we show that quasi-proportional FPA has a PoA of $2$ for any number of bidders, without any assumptions. Both of these bypass lower bounds in the deterministic setting. Finally, we study the setting where bidders are assumed to bid uniformly. We show that uniform bidding can be detrimental for efficiency in deterministic mechanisms while being beneficial for randomized mechanisms, which is in stark contrast with the settings without budget constraints.

==> scratchpad.tex <==
\section{Scratchpad}
This is mostly just scratchpad.

For rFPA, we consider two advertisers which we denote by $1$ and $2$.
Fix an equilibrium $\Eq$.

Let $\Opt_1$ be the contribution of advertiser $1$ to the optimal liquid welfare (and similarly for $\Opt_2$).
Similarly for $\LW_1, \LW_2$ for liquid welfare.
\paragraph{Case 1: Both advertisers are BC.}
This case is trivial.

\paragraph{Case 2: Advertiser $1$ is BC but advertiser $2$ is not.}
For this, we consider two sub-cases.

\paragraph{Case 2a: there exists query $j$ such that $b_{1,j} \geq \alpha \cdot (B_2 - \Veq_2)$.}
We are assuming advertiser $1$ is BC so $\LW_1 \geq \Opt_1$.
The assumption gives that $\Spend(j) \geq \alpha(B_2 - \Veq_2)$.
Hence, $\LW_1 + \frac{1}{\alpha} \Spend(j) \geq \Opt_1 + B_2 - \Veq_2$.
We conclude that $(1+1/\alpha) \LW \geq \Opt$, i.e.~$\LW \geq \frac{1}{1+1/\alpha} \cdot \Opt$.

\paragraph{Case 2b: there does not exist a query $j$ such that $b_{1,j} \geq \alpha \cdot (B_2 - \Veq_2)$.}
In this case, we still have $\LW_1 \geq \Opt_1$.

\paragraph{Case 3: Both advertisers are not BC.}
\paragraph{Case 3b:} In this case, we assume there exists $j^*$ such that $b_{1,j^*} \geq \alpha \cdot (B_2 - \Veq_2)$ and that there does not exist any $j$ such that $b_{2,j} \geq \alpha \cdot (B_1 - \Veq_1)$, i.e.~$\Spend(j) \geq \alpha \cdot (B_1 - \LW_1)$.

We consider three disjoint sets of queries.
Let $Q_1 = \{j \,:\, b_{2,j} \geq \alpha \cdot v_{1,j} \}$, $Q_2 = \{j \,:\, b_{2,j} / b_{1,j} \in (1/\alpha, \alpha)\}$ and $Q_3 = \{j \,:\, b_{2,j} / b_{1,j} \leq 1/\alpha\}$.
Note that $j^* \in Q_3$ so we do have to be mindful not to double count the spend on $j^*$.


